Steep Balmer decrement in weak AGNs may be not caused by dust extinction: clues from low-luminosity AGNs and changing-look AGNs

The hydrogen Balmer decrement (e.g., $\rm H\alpha/H\beta$) is widely adopted as an indicator of the internal reddening of active galactic nuclei (AGNs). This is challenged by some low-luminosity AGNs (LLAGNs) and changing-look AGNs (CLAGNs), which have steep Balmer decrement but without strong evidence for absorption. We compile a sample of normal AGNs and CLAGNs with a wider distribution of bolometric Eddington ratio ($\lambda_{\rm Edd}=L_{\rm bol}/L_{\rm Edd}$) and find a strong negative correlation between $\rm H\alpha/H\beta$ and $\lambda_{\rm Edd}$, which suggests that the Balmer decrement is also accretion-rate dependent. We further explore the Balmer decrement based on the photoionization model using the Cloudy code by considering spectral energy distribution (SED) from the accretion disk with different accretion rates (e.g., disk/corona and truncated disk at high and low Eddington ratios, respectively). Both the standard disk and truncated disk predict a negative correlation of $\rm H\alpha/H\beta-\lambda_{\rm Edd}$, where the relation is steeper in the case of the truncated disk. The negative correlations are also explored in two single CLAGNs. The measured negative correlation of $\rm H\alpha/H\beta$ -- $\lambda_{\rm Edd}$ is mainly caused by the lower responsivity $({\rm dlog}L_{\rm line}/{\rm dlog}L_{\rm cont})$ in $\rm H\alpha$ relative to that in $\rm H\beta$, due to the larger optical depth in the former. We propose that the steep Balmer decrements in low-Eddington-ratio AGNs (e.g., some Seyferts 1.5-1.9 and CLAGNs) are not simply caused by absorption but mainly caused by the relatively low flux of ionizing photons.

==> comment.tex <==



%1ES 1927+654 is also a TDE candidate  %Comments by lyubing



%The mass of single AGNs selected from \citep{Jin2022}, \citep{LaMura2007} are from the papers themselves.

%\textcolor{red}{One object with a very heavy SMBH $ {\rm log} ( M _{\rm BH}/ M _{\odot})=9.4 \pm 0.5$ from \cite{Onken2022} is also included, which can shed light on the possible affection by mass on the Balmer decrement.} And we rule out the observations lacking broad Balmer lines.


%active galactic nuclei (AGNs)
%active galactic nucleus (AGN)


%In this work, we make use of Ferland's spectral synthesis code CLOUDY version 17.03 to simulate the process occurring in the BLR cloud \citep{Ferland2017}. 


%\textcolor{red}{The average logarithmic mass of our sample is 7.18 with standard deviation 0.69 }.
w

%\textcolor{red}{It is interesting to point out that $\rm H\alpha/H\beta=5.2$ in SMSS J114447.77-430859.3, which possesses a BH with mass of $10^{9.4\pm 0.5}M_{\odot}$ and a bolometric Eddington ratio of 1.4. More observations with such high BH mass of AGNs can further test this scenario, which will be our following work.}

